Z3str3: A String Solver with Theory-aware Branching

We present a new string SMT solver, Z3str3, that is faster than its competitors Z3str2, Norn, CVC4, S3, and S3P over a majority of three industrial-strength benchmarks, namely Kaluza, PISA, and IBM AppScan. Z3str3 supports string equations, linear arithmetic over length function, and regular language membership predicate. The key algorithmic innovation behind the efficiency of Z3str3 is a technique we call theory-aware branching, wherein we modify Z3's branching heuristic to take into account the structure of theory literals to compute branching activities. In the traditional DPLL(T) architecture, the structure of theory literals is hidden from the DPLL(T) SAT solver because of the Boolean abstraction constructed over the input theory formula. By contrast, the theory-aware technique presented in this paper exposes the structure of theory literals to the DPLL(T) SAT solver's branching heuristic, thus enabling it to make much smarter decisions during its search than otherwise. As a consequence, Z3str3 has better performance than its competitors.

==> preliminaries.tex <==
\label{sec:preliminaries}

In this section, we briefly describe the input format accepted
by \toolname{}.  A more complete presentation of this language and the
corresponding logical theory is given in~\cite{cav15}.

The \toolname{} solver accepts input in the SMT-LIB
format~\cite{SMTLIB2} and can handle string and integer terms. The
syntax for string terms is compatible with other solvers such as CVC4
and Norn, and is in the process of standardization.  Terms that are
handled by the string solver may be either string terms, regular
expression terms, or integer length terms. Regular expressions are
constructed inductively and support standard operators including
concatenation, union, and Kleene star.  Some higher-level string
operators such as \textsf{indexof}, \textsf{contains},
and \textsf{charat} are also supported; these are rewritten to a
combination of string and length constraints.

For a string term $w$, $len(w)$ denotes the length of $w$ as an
integer number of characters.  The empty string $\epsilon$ has a
length of 0. String constants are composed of a finite sequence of
ASCII characters.


==> related.tex <==
Zheng et al. \cite{cav15} present the Z3str2 solver upon which this
work is based. The main difference between \toolname{} and its
predecessors is theory-aware branching and theory-aware case
splitting. The S3~\cite{s3} solver has similar capabilities and is
based on Z3-str (the predecessor to Z3str2). CVC4 \cite{CVC4-CAV14}
handles constraints over the theory of unbounded strings with length
and regex membership, and is also a DPLL($T$) solver.
Norn~\cite{norn} is based on a reduction from strings constraints to
Presburger arithmetic.


==> syntax.tex <==

\begin{figure}[t]
\centering
  \begin{tabular}{ lrl }
  {\it Term:bool} & ::= $~~~~$ & {\it Var:bool} \\
          & $|$  & {\sf true} \\
          & $|$  & {\sf false} \\
          & $|$  & ({\sf Contains} ~ {\it Term:string} ~ {\it Term:string})  \\ 
          & $|$  & ({\sf StartsWith} ~ {\it Term:string} ~ {\it Term:string})  \\
          & $|$  & ({\sf EndsWith} ~ {\it Term:string} ~ {\it Term:string})  \\        
          & $|$  & ({\sf RegexIn} ~ {\it Term:string} ~ {\it Term:regex}) \\        
          
  % int term
  {\it Term:int} & ::= $~~~~$ & {\it Var:int}  \\
          & $|$  & {\it Number} \\
          & $|$  & ($\{+, -, \times, \div\}$ ~ {\it Term:int} ~ {\it Term:int}) \\
          & $|$  & ({\sf Length} ~ {\it Term:string}) \\ 
          & $|$  & ({\sf IndexOf} ~ {\it Term:string} ~ {\it Term:string}) \\   
          & $|$  & ({\sf IndexOf2} ~ {\it Term:string} ~ {\it Term:string} ~ {\it Term:int}) \\           
          & $|$  & ({\sf LastIndexOf} ~ {\it Term:string} ~ {\it Term:string}) \\
              
  % string term
  {\it Term:string} & ::= $~~~~$ & {\it Var:string}  \\
          & $|$  & {\it ConstStr} \\
          & $|$  & ({\sf Concat} ~ {\it Term:string} ~ {\it Term:string}) \\ 
          & $|$  & ({\sf Substring} ~ {\it Term:string} ~ {\it Term:int} ~ {\it Term:int}) \\   
          & $|$  & ({\sf Replace} ~ {\it Term:string} ~ {\it Term:string} ~ {\it Term:string}) \\
          & $|$  & ({\sf CharAt} ~ {\it Term:string} ~ {\it Term:int}) \\   

  % regex
  {\it Term:regex} & ::= $~~~~$ & ({\sf Str2Regex} ~ {\it ConstStr:string}) \\
          & $|$  & ({\sf RegexStar}  {\it Term:regex} ) \\
          & $|$  & {\it (Term:regex)+}  \\
          & $|$  & {\it (Term:regex)?}  \\
          & $|$  & ({\sf RegexConcat} ~ {\it Term:regex} ~ {\it Term:regex})\\ 
          & $|$  & ({\sf RegexUnion} ~ {\it Term:regex} ~ {\it Term:regex})\\ 

  %
  {\it Expr:bool}       & ::=  $~~~~$ & {\it Term:bool} \\
          & $|$  & ($=$ ~ {\it Term:bool} ~ {\it Term:bool}) \\ 
          & $|$  & ({\sf not} ~ {\it Expr:bool})  \\
          & $|$  & ({\sf and} ~ {\it Expr:bool} ~ {\it Expr:bool}) \\
          & $|$  & ({\sf or} ~ {\it Expr:bool} ~ {\it Expr:bool}) \\
          & $|$  & ({\sf ite} ~ {\it Expr:bool} ~ {\it Expr:bool} ~ {\it Expr:bool})\\
          & $|$  & ({\sf implies} ~ {\it Expr:bool} ~ {\it Expr:bool}) \\
          & $|$  & ($\{<, \leq, =, \geq,>\}$ ~ {\it Term:int} ~ {\it Term:int}) \\                
          & $|$  & ($=$ ~ {\it Term:string} ~ {\it Term:string})\\        
          
  {\it Assertion}     & ::= $~~~~$  &  ({\bf assert} ~ {\it Expr:bool} ) \\
  \end{tabular}
\caption{Constraint syntax}
\label{fig:language}
\end{figure}


